TAR3D: Creating High-Quality 3D Assets via Next-Part Prediction

We present TAR3D, a novel framework that consists of a 3D-aware Vector Quantized-Variational AutoEncoder (VQ-VAE) and a Generative Pre-trained Transformer (GPT) to generate high-quality 3D assets. The core insight of this work is to migrate the multimodal unification and promising learning capabilities of the next-token prediction paradigm to conditional 3D object generation. To achieve this, the 3D VQ-VAE first encodes a wide range of 3D shapes into a compact triplane latent space and utilizes a set of discrete representations from a trainable codebook to reconstruct fine-grained geometries under the supervision of query point occupancy. Then, the 3D GPT, equipped with a custom triplane position embedding called TriPE, predicts the codebook index sequence with prefilling prompt tokens in an autoregressive manner so that the composition of 3D geometries can be modeled part by part. Extensive experiments on ShapeNet and Objaverse demonstrate that TAR3D can achieve superior generation quality over existing methods in text-to-3D and image-to-3D tasks

==> figs/intro.tex <==




\twocolumn[{%
    \renewcommand\twocolumn[1][]{#1}%
    \maketitle
    \vspace{-25pt}
    \begin{center}
      \captionsetup{type=figure}   
      \footnotesize
      % \fbox{\rule{0pt}{2.3in} \rule{0.9\linewidth}{0pt}}
       \includegraphics[width=0.97\linewidth]{figs/files/gallery3.pdf}
      \captionof{figure}{
        Examples of high-quality 3D asset gallery generated by our \ourMthd{} model.
        % 
        We employ SyncMVD~\cite{liu2024text} as the texture synthesizer.
      }
      \label{fig:intro}
      \vspace{3pt}    
    \end{center}%
}]  

==> figs/suppl_ito3d.tex <==

% \clearpage
\begin{figure*}[htbp]
  \centering
  \footnotesize
  % \fbox{\rule{0pt}{4in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=\linewidth]{figs/suppl_files/suppl_ito3d.pdf}

   \caption{Given a wide range of input images from the benchmark datasets, \ie ShapeNet and Objaverse, our \ourMthd{} model is capable of inferring the full picture of the primary objects and producing high-quality 3D meshes that adhere to them.}
   \label{fig:suppl_ito3d}
\end{figure*}
% \clearpage
% \raggedbottom

% \renewcommand{\floatpagefraction}{1.0}
% \renewcommand{\textfraction}{0.0}

% \WarningFilter{latex}{Text page contains only floats} % 忽略特定警告

==> figs/suppl_ito3d_gso.tex <==

% \clearpage
\begin{figure*}[htbp]
  \centering
  \footnotesize
  % \fbox{\rule{0pt}{4in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=\linewidth]{figs/suppl_files/suppl_ito3d_gso.pdf}

   \caption{Given a wide range of input images from the out-of-domain dataset, \ie GSO, our \ourMthd{} model is capable of inferring the full picture of the primary objects and producing high-quality 3D meshes that adhere to them.}
   \label{fig:suppl_ito3d_gso}
\end{figure*}
% \clearpage
% \raggedbottom

% \renewcommand{\floatpagefraction}{1.0}
% \renewcommand{\textfraction}{0.0}

% \WarningFilter{latex}{Text page contains only floats} % 忽略特定警告

==> figs/suppl_tto3d.tex <==
\begin{figure*}[t]
  \centering
  \footnotesize
  % \fbox{\rule{0pt}{4in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=.98\linewidth]{figs/suppl_files/suppl_tto3d.pdf}

   \caption{Qualitative results of our \ourMthd{} on a broad spectrum of text prompts.
   %
   It can be observed that these 3D meshes created by our \ourMthd{} model are semantically faithful to the textual descriptions.
   }
   % \vspace{-5pt}
   \label{fig:suppl_tto3d}
\end{figure*}

==> tabs/abl_pii.tex <==
\begin{table}[tp]
\setlength\tabcolsep{19pt}
\centering
\footnotesize
\caption{Ablation studies on the PII design of the 3D-VQVAE.
} 
\vspace{-7pt}
\begin{tabular}{lcc}
\toprule
& \emph{w/o} PII & \emph{w/} PII  \\  
\midrule 
Chamfer Distance~$\downarrow$ & 0.023  &  0.016   \\
\midrule 
 F-Score~$\uparrow$ & 0.661 & 0.822  \\
\bottomrule
\end{tabular}
\vspace{-3pt}
\label{tab:abl_pii}
\end{table}


==> tabs/abl_triplanesize.tex <==
\begin{table}[tp]
\setlength\tabcolsep{6pt}
\centering
\footnotesize
\caption{Ablation studies on triplane size of the 3D GPT.
} 
\vspace{-7pt}
\begin{tabular}{lccc}
\toprule
Triplane Size & $3 \!\times\! 16 \!\times\! 16$ & $3 \!\times\! 32 \!\times\! 32$ & $3 \!\times\! 48 \!\times\! 48$ \\    
\midrule 
Chamfer Distance~$\downarrow$  & 0.157  &  0.066 & 0.062 \\
\midrule 
Inference Time~$\downarrow$  &  17.7~s &  67.6~s & 143.9~s\\
\bottomrule
\end{tabular}
\vspace{-3pt}
\label{tab:abl_triplanesize}
\end{table}

